GOPO: Policy Optimization using Ranked Rewards

Standard reinforcement learning from human feedback (RLHF) trains a reward model on pairwise preference data and then uses it for policy optimization. However, while reward models are optimized to capture relative preferences, existing policy optimization techniques rely on absolute reward magnitudes during training. In settings where the rewards are non-verifiable such as summarization, instruction following, and chat completion, this misalignment often leads to suboptimal performance. We introduce Group Ordinal Policy Optimization (GOPO), a policy optimization method that uses only the ranking of the rewards and discards their magnitudes. Our rank-based transformation of rewards provides several gains, compared to Group Relative Policy Optimization (GRPO), in settings with non-verifiable rewards: (1) consistently higher training/validation reward trajectories, (2) improved LLM-as-judge evaluations across most intermediate training steps, and (3) reaching a policy of comparable quality in substantially less training steps than GRPO. We demonstrate consistent improvements across a range of tasks and model sizes.

==> grpo-rank/archive/experiments.tex <==
\section{Experiments}
We fix 
\begin{itemize}
    \item $\pi_{\theta_0}$: Llama 8B or Distilled R1 
    \item $r_\phi$: QRM (Quantile reward model) \cite{dorka2024quantile} --- outputs not only the mean response, but also the quantile values of the response distribution. 
\end{itemize}


Let $\hat o_k^{(b, j)} = |o_k^{(b, j)}|^{-1}\sum_{\ell}^{|o_k^{(b, j)}|} h( o_{k, \ell}^{(b, j)} )$ be the averaged hidden state of the output across its tokens, where $o_{k, \ell}^{(b, j)}$ is the $\ell$th token of the output $o_k^{(b, j)}$. For the $b'$th step of training, use labeled data $\{o_k^{(b, j)}, r_k^{(b, j)}\}_{k \in [N], j \in [n], b \in [b' - 1]}$ to train a regression model $\hat f$. Then approximate $r_k^{(b, j)}$ by $\hat r_k^{(b, j)} = \hat f (p_j^{(b)}, o_k^{(b, j)})$.


The goal here is to understand the source of bias when regression techniques are used and to investigate ways to debias. Here, we rely heavily on the oracle reward hence deviating from our initial spirit---we intend to provide a proof of concept, that regression methods are useful tools to approximate policy updates. An implementable~(i.e. minimal oracle calling) regression based algorithm is to be investigated in the next section. 

% the bias from regression affect our end goal, which is to maximize true reward of the outputs generated by the updated policy. 

\subsection{Source of bias} Here we analyze why the metric trajectory deviates from the oracle when regression model is used fully. Refer to Figure \ref{fig:Bias} to observe the bias occuring by resorting purely to regression for the later training steps. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figure/oracle_and_full.png}
    \caption{Caption}
    \label{fig:Bias}
\end{figure}

The bias is essentially coming from the consistent update of the policy. Note that we may take either of the two approaches to address the bias: \textit{Debiasing} or \textit{Online learning}. The first approach we use the technique `patching' and the second we use online regression.


\subsection{Approach 1: Patching}

We conjecture that policy optimization~(GD of KL-penalized objective functions) are robust to the magnitude of reward values, as long as the orders or the rewards across outputs are retained. So we measure the ordering between forecasted rewards and the oracle rewards of the outputs per prompt, then the measure is used for a decision rule on whether or not the forecasted reward should be used~(i.e. patching). 

Fix $b \in [B]$ and the corresponding batch of queries $\mc D_b = \{p_1^{(b)}, ..., p_n^{(b)}\}$, define the correlation between the oracle and estimated rewards per query, i.e.
\begin{equation*}
    \rho^{(b)}_j := \mathsf{Corr}\big( r_{1:N}^{(b, j)}, \hat r_{1:N}^{(b, j)} \big).
\end{equation*}
Higher correlation $\rho^{(b)}_j$ implies that the oracle and forecasted reward well aligns, implying that forecasted reward may substitute the oracle when updating policy. So for constructing objective function at step $b$, we feed forecasted reward into the objective for those outputs whose correlation is positive. Otherwise we feed the oracle reward. See the \textcolor{red}{red} trajectory to see the performance of the patching algorithm. Note that $\rho^{(b)}_j$ can only be computed with access to the oracle rewards.

\subsubsection{Specifics of experiment}

The \textcolor{green}{green} trajectory results from the following:
\begin{enumerate}
    \item Use the reward / output pair from the first $50$ training steps to train a linear regression model taking the hidden state of the outputs as the feature and the reward as response.
    \item Starting from the $51$st training step, the objective function takes in the estimated reward, which is simply the predicted response of the linear regression model for every hidden state of the output generated from the previous policy. 
\end{enumerate}

The \textcolor{red}{red} trajectory results from the following:
\begin{enumerate}
    \item Use the reward / output pair from the first $50$ training steps to train a linear regression model taking the hidden state of the outputs as the feature and the reward as response.
    \item Starting from the $51$st training step, the objective function takes in a mixture of estimated and true reward. Correlation between the true and estimated reward is calculated per prompt~($8$ outputs per prompt). Whenever correlation is positive for a specific prompt, the estimated rewards are used for the outputs. Otherwise the true rewards are used for the objective function. 
\end{enumerate}

\subsubsection{Observations from experiment}
\begin{itemize}
    \item True reward is \textit{not} called after $51$th training step for the \textcolor{green}{green} trajectory/
    \item True reward \textit{is} called after $51$th training step for the \textcolor{red}{red} trajectory in order to calculate the correlation.
    \item The \textcolor{green}{green} trajectory exhibits a systematic bias from the oracle~(\textcolor{blue}{blue} line) which is expected. However, the bias does not seem to occur up to around $80$th training steps. 
    \item The \textcolor{red}{red} trajectory seems to adjust for the systematic bias.
\end{itemize}


So we may infer:
\begin{itemize}
    \item Estimating the correlation per prompt without calling the true reward model would be a way to adjust for the bias in a fully data dependent manner
    \item An online linear regression, which updates the estimated coefficient, could be another way to adjust for the bias. Refer to \href{https://huggingface.co/learn/deep-rl-course/en/unit3/deep-q-algorithm}{deep Q-learning} technique.
\end{itemize}

\subsection{Approach 2: Online regression}

\textcolor{red}{TODO: not even sure if this would be of interest here; but if so, will be implemented much later. }

\newcommand{\gptfour}{\texttt{gpt4}}
\newcommand{\gptfouro}{\texttt{gpt4-o}}
\newcommand{\sonnetthreefive}{\texttt{sonnet3.5}}
\newcommand{\referencepolicy}{\texttt{Qwen2.5-1.5B-Instruct}}
\newcommand{\oraclemodel}{\pi_{\mrm{oracle}}}
\newcommand{\imputeoraclemodel}{\pi^\star_{\mrm{impute}}}
\newcommand{\basemodel}{\pi_{\mrm{ref}}}

\subsection{LLM as judge}
Three updated policies are compared using three different judges: $\gptfour, \gptfouro, \sonnetthreefive$. The updated policies start from the reference policy $\referencepolicy$, and all updates follow the GRPO style objective function; the difference comes from how the rewards are computed at each training step ($300$ steps total) with the \textcolor{red}{same tuning parameter $\beta$ assigned for the KL-divergence from the reference policy $\basemodel$ (@WK: let's verify that this is true?)}.
\begin{itemize}
    \item $\oraclemodel$: the policy is trained with the `true' reward model (cite, the quantile based reward model specialized for ultrachat dataset), 
    \item $\imputeoraclemodel$: the policy is updated according to the `true' reward model up to $0.2$th portion of the total update steps (here $80$ steps in total). Then regression model is trained on the data collected from the initial $80$ update steps, from which predicted rewards are calculated. `True' rewards are still queried throughout for the calculation of the correlation between the `true' rewards and the predicted rewards. If the \textcolor{red}{correlation}\footnote{We initially calculated this measure by an internal metric (inverse probability of token generation? so as to measure the confidence) --- we'll have to look into other metrics as well.} is positive, then predicted reward is used, otherwise `true' reward is used. 
\end{itemize}


\begin{table}[h]
\centering
\begin{tabular}{lcc}
& \textbf{$\basemodel$ vs. $\imputeoraclemodel$} & \textbf{$\imputeoraclemodel$ vs. $\oraclemodel$} \\[0.5ex]
\textbf{$\sonnetthreefive$} & $0.25$ / $0.72$ & $0.5$ / $0.5$ \\
\textbf{$\gptfouro$} &  &  \\
\textbf{$\gptfour$} &  &  \\
\end{tabular}
\caption{Your table caption here}
\label{tab:your_label}
\end{table}

\subsection{LLM as Judge - v2s}

Here, we consider a policy that still uses the regression, but the threshold for employing regression based rewards into the object function depends on the \textit{metric of confidence}.

\subsection{Linearly projected reward proxy as a self-regularizer}

The linear regression approach learns from the \textit{initial few step} completion/reward samples, so the completions that were used for constructing the linear reward does not exhibit distributional shifts (whatever this means). \textcolor{red}{Then can linearly distilled reward models serve as natural regularizers? Would it overcome some of the tuning-parameter engineering issues, by providing a more principled and robust method of avoiding the update to drastically shift from the reference models? An interesting experiment setup would be to update policies with a new objective function where KL divergence vanishes but only uses the linear regression rewards after the initial training steps... so the first $0.2$ portion (can we make the portion smaller?) requires KL divergence as training samples are collected, then we } 


I don't know how the reward models are usually trained, but is it the case that they are trained on a local set of samples, so that the trained model tends to overfit several niche areas? If so, the linearity would smooth out the reward plane. 






\subsection{Various definitions for the confidence of policy, and a unified view}

Consider the line of literatures that updates policies without referring to external reward models, \cite{zhang2025right, zhao2025learning}. The internal signals all have some meaningful correlations with the \textit{notion of variance} of the outputs of the policies. What if we measure the confidence of the policy in terms of the variance of the outputs (in GRPO, when normalizing, the variance of the reward is considered, which is a different object). 






==> grpo-rank/archive/intro.tex <==
\section{Introduction}



\paragraph{Definition of over-optimization in both RLHF and DAA style post-training}

We review literature that circumvents heavy use of reward models when post-training a language model. 

Over-optimization of rewards (i.e. reward hacking) refers to a deterioration or plateau of model performance during training, while the reward evaluated for the updated policies increase. The objective function of policy optimization (PO) takes the external reward model, hence the possibility of reward hacking is expected, as the actual metric we would like is the objective quality of the updated policies. 

From \cite{rafailov2024scaling}, 

\paragraph{Conjectures on why over-optimization occurs}

For simplicity, let $\mc L_X$ be the distribution of prompts $\{x_1, ..., x_n\}$ and $\pi_{\mrm{ref}}$ be the reference policy (mostly supervised-fine-tuned, or SFT) that follows distribution $\mc L_{\mrm{ref}}$. From the prompts and the reference policy, triples $(x_i, y_{i, 1}, y_{i, 0}) \sim \mc L_X \times \mc L_{\mrm{ref}}$ are generated. Until now, no true (i.e., human-like) distribution information is encoded. 

Using the information sampled from distribution $\mc L_X \times \mc L_{\mrm{ref}}$, an external true disribution $\mc L_\star$ is injected via two `models': the reward model $r_\phi$ and Bradley-Terry model; $r_\phi$ parametrizes the reward an answer receives given a promopt and BT model parametrizes how human choose one answer over the other. The trained reward model $r_\phi$ (we put no distinction between the model and the trained) hence encodes distribution $\mc L_X\times \mc L_{\mrm{ref}}\times \mc L_\star$ in an \textit{approximate manner.} 

When training, each optimization step uses different set of prompts. Assuming that the prompts are randomly sub-sampled from a population, the prompt distribution $\mc L_X$ remains unchanged throughout the training process. Consider some point during the training process and where prompts are fed onto the current policy $\pi_1$ that follows distribution $\mc L_1$. Then for a prompt $x \sim \mc L_X$, $\pi_1$ generates a response, which in turn is evaluated by the reward $r_\phi$. The objective function hence has the following dependency
\begin{align}
    \mc J = \mc J(\mc L_X, \mc L_{\pi_1}, \mc L_{\mrm{ref}}, \mc L_\star)
\end{align}

Within the RLHF training process, 


To address the problem of over-optimization of RLHF type policy update and the cost of human labels, verifiable rewards, two approaches have been introduces: (i) creating pseudo data points leveraging the `true' reward models to some extent, (ii) utilizing model's internal signal, hence no leverage of the `true' reward model.


\paragraph{Policy update by pseudo-data}



\paragraph{Policy update by internal signals}

Two interesting implications: either that (i) model is not knowledgeable enough to know the answer, but when identifying the problem, it is capable of learning by itself, or (ii) there exists an internal signal that correlates with the correctness indicated by the reward model... so the model is indeed knowledgeable, and the problem is finding the number that signifies such information.



Previously, we used a measure of confidence (@WK what was it? the inverse probability of the output?) within the learning procedure---if the model is confident, then use regression, otherwise use the reward model to incorporate edge case information. 




We are using correlation... this is first order information, should we also try using the KL divergence??? 


Self consistency... the KL divergence between the output distribution of the model and the uniform distribution --- the more prominent the spike of output distribution, the more confident on the answer. This idea essentially connect to the variance of the output distribution. Is Wasserstein computation of a distribution to uniform easy? 

The objective function for updating the policies reinforces confidence of a model (i.e. encouraging the model to reason through paths that its understands better, hence more confident about):
\begin{enumerate}
    \item is this based on the observation (exactly referred where and how? see Kang et al., 2025) that confidence and correctness is correlated? Such interpretation is subtly assuming that the model already knows the answers, and all the post-training has to do is to point towards the location within the model where the answers are. 
    \item is this based on the idea that regardless of correctness, following the most confident path eventually leads to a correct answer? It's as if you're nurturing a capable child, for it to explore and identify the right with confidence... this is about meaningful progress. 
\end{enumerate}

\textcolor{red}{If we learn a logistic regression model for verifiable reward settings, then can the learned probability serve as a proxy for confidence?}



There is the distribiution shift problem in policy optimization where the completions of moving policies are evaluated on a static reward model




==> grpo-rank/archive/method.tex <==
\section{Method}

\subsection{GRPO}

Consider a single epoch training scheme, and let's redefine definitions. From RewardBench~\cite{lambert2024rewardbench}, we use the `chat' data set consisting of $358$ triples of prompt, chosen / rejected outputs, say $(p, o_1, o_2)$ with additional information on which of the two $o_1, o_2$ are preferred over the other. 

\begin{itemize}
    \item $b \in [B]$: index of training stedps
    \item $j \in [n]$: index of the prompts within the batch of prompts assigned to each training steps
    \item $k \in [N]$: index of the outputs generated by a policy and a prompt
\end{itemize}

Let $\mc D_b= \{ p_1^{(b)}, ..., p_n^{(b)} \}$ for $b = 1, ..., B$ be the batches of the prompts~(questions). Let $\pi_{\theta_b}$ for $b = 0, ..., B$ be the sequence of policies where $\pi_{\theta_0}$ is the starting policy~(post-SFT) and $\pi_{\theta_b}$ is updated at the $b$th training step and let 
\begin{equation*}
    o_1^{(b, j)}, ..., o_N^{(b, j)} \sim \pi_{\theta_b}(\cdot | p_j^{(b)})
\end{equation*}
be the $N$ number of outputs~(of all different token lengths) generated by policy $\pi_{\theta_b}$ and prompt $p_j^{(b)}$---for any output $o$ of token length $|o|$, let $h(o)$ be an $|o| \times H$ sized matrix, where each column is the hidden state of dimension $H$ for each tokens of $o$. For some fixed reward model $r_\phi$, let
\begin{equation*}
    r_{k}^{(b, j)} = r_\phi(p_j^{(b)}, o_k^{(b, j)})
\end{equation*}
be the reward called for prompt $p_j^{(b)}$ and output $o_k^{(b, j)}$.

\begin{equation*}
    \textbf{(Goal): Forecast rewards $r_k^{(b, j)}$ by regression $\hat r_k^{(b, j)} = \hat f (p_j^{(b)}, o_k^{(b, j)})$.}
\end{equation*}



\subsection{Smart Search}

Let $\mc E$ be the embedding model for whatever string $\mathsf{T}$ that is observed, $\mc E : \mathsf{T} \mapsto \mathbb{R}^d$. We use an external embedding model for the sub-queries and the sub-answers as hidden states are difficult to extract from a VLLM~(needed for fast inference) transformer architecture. Also we already have access to the embeddings of the wikipedia pages $w_{d, j}$ for all $j = 1, ..., J$ and $d = 1, ..., D$ provided by the CoRAG agent. So with abuse of notation, we regard $w_{d, j}, w_d, w_{1:d}$ both as the text and its (collection of) embeddings.

Each query~(question to answer) is indexed by $i\in [n]$ and per query, 
\begin{equation*}
    s_d^{(i)}, s_{1:d}^{(i)}, a_d^{(i)}, a_{1:d}^{(i)}, w_d^{(i)}, w_{1:d}^{(i)}, c_{i, d}
\end{equation*}
refer to the trace of the \textit{trajectory selected by the tree search algorithm.} For any two texts $a, b$, define operation $a \oplus b$ as the simple concatenation (with space, with comma). Define 
\begin{equation*}
    \mathsf{(s*a)_d^{(i)}} = s_{1}^{(i)} \oplus a_1^{(i)} \oplus s_2^{(i)} \oplus a_2^{(i)} \oplus ... \oplus s_d^{(i)} \oplus a_d^{(i)}
\end{equation*}
as the concatenation of sub-query, sub-answer pairs. We do the following:
\begin{enumerate}
    \item (\textit{feature engineering}) For each query $i \in [n]$ and depth $d \in [D]$, embed the concatenated vector of sub-query / sub-answer texts so we have $ \mc E \big\{ ( \mathsf{s*a} )_d^{(i)} \big\}$. Next concatenate the embedding with the averaged wikipedia embeddings $\overline w^{(i)}_d = J^{-1}\sum_{j = 1}^{J}w_{j}^{(d)}$,
    \begin{equation*}
        X_{i, d} := \big[ \mc E \big\{ ( \mathsf{s*a} )_d^{(i)} \big\}, \overline w^{(i)}_d \big].
    \end{equation*}
    \item (\textit{train regression model(s)}) Either attain 
    \begin{equation*}
        \begin{aligned}
            \hat \beta & \stackrel{\mathrm{LR}}{\longleftarrow} \big\{ c_{i, d}, X_{i, d}: i \in [n], d \in [D] \big\}\\
            \hat \beta^d& \stackrel{\mathrm{LR}}{\longleftarrow} \big\{ c_{i, d}, X_{i, d}: i \in [n]\big\} \quad \text{for all $d \in [D]$}.
        \end{aligned}
    \end{equation*}
    $\hat \beta$ \textit{averages} the autoregressive information across the depth $d \in [D]$, whereas $\hat \beta^{d}$ doesn't. For simplicity, we stick to using a single linear model $\hat \beta$.
    \item (\textit{test estimated penalty}) In the test data set, replace the penalty of the tree search algorithm to the estimated one using $\hat \beta$, embeddings of sub-query / sub-answer pair and the embeddings of the retrieved documents. 
\end{enumerate}


==> grpo-rank/archive/review.tex <==
\section{Overview}

\subsection{GRPO}

We first review the GRPO algorithm in \cite{shao2024deepseekmath}. Given a sampled prompt $q \sim P_Q$, let $o_i = [o_{i, 1}, ..., o_{i, T}]$ for $i = 1, ..., G$ be the response generated from the \textit{old} policy $\pizero(\cdot|q)$. Define the shorthand $o_{1:s} = \{ o_1, ..., o_s \}$ for any $s \in [T]$, and for any fixed response $i$ and its $t$th token,
\begin{equation}
    \pi_t(\theta|\theta_0) := \frac{\pi_\theta(o_{i, t}|q, o_{1:t - 1})}{\pizero(o_{i, t}|q, o_{1:t - 1})}.
\end{equation}
The objective function of GRPO is
\begin{equation*}
    \begin{aligned}
        &\mc J_{\mathrm{GRPO}}(\theta)\\
        &= \E_{q \sim P_Q, o_{1:T} \sim \pizero(\cdot|q)}\bigg[ \frac{1}{G}\sum_{i = 1}^{G} \frac{1}{T}\sum_{t = 1}^{T} \min\Big\{ \pi_t(\theta|\theta_0)\hat A_{i, t}, \mathrm{clip}(\pi_t(\theta|\theta_0), 1 - \varepsilon, 1 + \varepsilon)\hat A_{i, t} \Big\} - \beta \mathrm{KL}( \pi_\theta \| \piref ) \bigg].
    \end{aligned}
\end{equation*}
The approximated advantage $\hat{A}_{i, t}$ is the innovative aspect. Notice $\piref$ is the reference policy, usually set as the initial SFT model.


Let $\mc D$ be the population of prompts and for $b \in [B]$, let the batch be $\mc D_b \subset \mc D$. Overall, the training procedure (i) fixes the reference policy $\piref$~(so the KL divergence part of $\mc J_{\mathrm{GRPO}}$ is fixed) as $\pione$, then (ii) sequentially optimize $\mc J_{\mathrm{GRPO}}$ for each batches $\mc D_b$ for $b = 1, ..., B.$ To be specific, start with $\pione$,
\[
\begin{array}{c}
\text{$(\star)$ For each $i$, fix $\piref^{(i)} \leftarrow \pione$} \\
\downarrow \\
\text{$(\star\star)$ For each $b$, select batch $\mc D_b = \{p_1, ..., p_K\}$ } \\
\downarrow \\
\text{Set $\pizero \leftarrow \pione$}\\
\downarrow\\
\text{For each prompt $p_k \in \mc D_b$, generate $o_1^{(k)}, ..., o_T^{(k)} \sim \pizero$ and evaluate $r_1^{(k)}, ..., r_T^{(k)}$ by $r_\varphi$}\\
\downarrow\\
\text{Construct the empirical~(w.r.t. prompt) version of $\mc J_{\mathrm{GRPO}}$ using $\mc D_b$, $\piref$, $o^{(k)}$ and $r^{(k)}$}\\
\downarrow\\
\text{Do gradient descent on the empirical version of $\mc J_{\mathrm{GRPO}}$ for $\mu$ times set the optimizer $\pione$}\\
\downarrow\\
\text{Until $b = B$, go back to $(\star\star)$}\\
\downarrow\\
\text{Until $i = I$, go back to $(\star)$}
\end{array}
\]
So there are four dimensions at play: $i\in[I]$ is the outer loop which updates the reference policy, $b \in [B]$ is the sequential update loop of the policy while fixing reference policy, and $K\times T$ matrix of prompt, reward combination. 

\subsection{PPO}




\subsection{Smart Search}

Every tree search method involves an extensive exploration along possible trajectories, the cost of exploration increasing significantly if roll-outs are implemented per node. The computational difficulty here is analogous to that of PPO, where value function estimation is required per token generation.

The goal is to approximate a searching algorithm while implementing it in a more efficient manner. 

% We expect efficiency can allow us to go deeper into the tree when needed, given an assigned budget. 

% So the tree depth can be limited when resource is scarce which may hinder accuracy. We 

We review the high-level procedure of the modified PHS + CoRAG algorithm. The specifics are to be further optimized, but the high-level procedure is sufficient to evaluate the proposed regression based searching.
\begin{itemize}
    \item (\textit{sub-queries}) Let $s_0$ be the initial query~(question we would like to answer) fed into the language model and $s_1, ..., s_{D}$ be the sequence of sub-queries generated by the tree algorithm. 
    \item (\textit{document retrieval}) At each depth $d$, wikipedia pages, say $w_{d, j}$ for $j = 1, .., J$, are retrieval for sub-query $s_d$.
    \item (\textit{sub-answers}) At each depth $d$, the  documents $w_d:= \{w_{d, j}, j \in [J]\}$ and the sub-query $s_d$ are passed through some function to generated sub-answer $a_d$. 
    \item (\textit{reward per depth}) At each depth $d$, history of sub-queries $s_{1:d}$, sub-answers $a_{1:d }$ and documents $w_{1:d}:=\{ w_{d} \}_{d' = 1, ..., d}$ are all combined to generate a penalty, say $c_d$. Node with the lowest penalty are chosen in the tree algorithm.
\end{itemize}

In short, there exists functions $\textcolor{red}{A}, C, \textcolor{blue}{S}$ such that
\begin{equation}
    \begin{aligned}
        a_d &\leftarrow \textcolor{red}{A}(s_{d}, w_d)\\
        c_{d} &\leftarrow C(s_{1:d}, a_{1:d})\\
        s_{d + 1} &\leftarrow \textcolor{blue}{S}(s_{d}, a_{d}).\\
    \end{aligned}
\end{equation}
The graph in Figure \ref{fig:dynamic} depicts a two step dynamic of $\textcolor{red}{A}, C, \textcolor{blue}{S}$. Our goal is to
\begin{equation}
    \textit{approximate function $C$ using regression.}
\end{equation}

\definecolor{offwhite}{HTML}{F2EDED}

\tikzset{
    > = stealth,
    every node/.append style = {
        text = black
    },
    every path/.append style = {
        arrows = ->,
        draw = black,
        fill = offwhite
    },
    hidden/.style = {
        draw = black,
        shape = circle,
        inner sep = 1pt
    }
}


\begin{figure}
\centering
\begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}]
\node[main] (1) {$s_1$}; 
\node[main] (2) [right of=1] {$a_1$};
\node[main] (4) [below right of=2] {$c_1$};
\node[main] (3) [above right of=4] {$w_1$};
\node[main] (6) [below left of=4] {$a_2$};
\node[main] (5) [left of=6] {$s_2$};
\node[main] (7) [below right of=4] {$w_2$};
\node[main] (8) [below right of=6] {$c_2$};

% first chunk
\draw[red] (1) -- (2);
\draw[red] (3) -- (2);
\draw (1) -- (4); % to cost
\draw (2) -- (4); % to cost
% \draw (3) -- (4); % to cost
% second chunk
\draw[red] (5) -- (6);
\draw[red] (7) -- (6);
\draw (5) -- (8); % to cost
\draw (6) -- (8); % to cost
% \draw (7) -- (8); % to cost
% first to second chunk
\draw[blue] (1) -- (5);
\draw[blue] (2) -- (5);
\draw (1) -- (8); 
\draw (2) -- (8);
% \draw (3) -- (8);
\end{tikzpicture}
\caption{\textcolor{red}{Red}, black, \textcolor{blue}{blue} lines corresponds to the mapping of functions $\textcolor{red}{A}$, C, $\textcolor{blue}{S}$ respectively.}
\label{fig:dynamic}
\end{figure}

